Integrated Sensing and Communication with MOCZ Waveform

In this work, we propose a waveform based on Modulation on Conjugate-reciprocal Zeros (MOCZ) originally proposed for short-packet communications in [1], as a new Integrated Sensing and Communication (ISAC) waveform. Having previously established the key advantages of MOCZ for noncoherent and sporadic communication, here we leverage the optimal auto-correlation property of Binary MOCZ (BMOCZ) for sensing applications. Due to this property, which eliminates the need for separate communication and radar-centric waveforms, we propose a new frame structure for ISAC, where pilot sequences and preambles become obsolete and are completely removed from the frame. As a result, the data rate can be significantly improved. Aimed at (hardware-) cost-effective radar-sensing applications, we consider a Hybrid Digital-Analog (HDA) beamforming architecture for data transmission and radar sensing. We demonstrate via extensive simulations, that a communication data rate, significantly higher than existing standards can be achieved, while simultaneously achieving sensing performance comparable to state-of-the-art sensing systems.

==> MOCZ_modulation.tex <==
\section{MOCZ Principles}\label{MOCZ_basics}
Among the main
challenges new emerging technologies have to cope with is the
support of a massive number (billions) of devices/machines ranging from powerful smartphones and tablet computers
to small and low-cost sensor nodes. These devices come
with diverse and even contradictory types of traffic including
high-speed cellular links, machine-to-machine (M2M) connections, and wireless links which carrying data in short-packets.
Such short messages of sporadic nature [1] will dominate
the future communication and the conventional cellular and
centrally-managed wireless network infrastructure will not be
flexible enough to keep pace with these demands. 


\subsection{BMOCZ with Huffman Sequences}\label{sec:huffman}
%
The proposed BMOCZ scheme can be applied to any given autocorrelation sequence $\av = \xv * \cc{\xv^-}\in\C^{2K+1}$
which will generate a polynomial of simple zeros (all zeros are distinct). The BMOCZ codebook consists
then of all non-trivial ambiguities $\xv\in\C^{K+1}$ of this particular autocorrelation \cite{WJPH16a}. Since, we
cannot use the global phase (trivial ambiguity) as an information resource in a non-coherent communication, we will
always choose the first coefficient $x_0$ to be positive.
%
However, among all such autocorrelations, \emph{Huffman autocorrelations} \cite{Huf62} posses three remarkable
properties, which renders Huffman  BMOCZ to a superior  MOZ design. 1.) Huffman
sequences have the most ``impulsive-like'' autocorrelation  2.) The zeros of their polynomials are evenly placed
on two reciprocal circles centered at the origin and 3.)  remain approximately unchanged if the polynomial
coefficients are disturbed by additive noise.  Let us begin with the first two properties and investigate the robustness
mathematically and numerically later on.  Huffman autocorrelations
%
\begin{align}
  \av=(a_0,0,\dots,0,a_K,0,\dots,0,a_{2K})^\tran\label{eq:huffmanauto}
\end{align}
%
are given by a central-peak $a_K=1$ and two side-peaks $a_0=-\eta=a_{2K}$ of magnitude $\eta\in (0,1/2)$.  Note, that unlike circular autocorrelations, the side-peaks can never vanish for sequences $\xv$ with non-vanishing first and last coefficients, since $a_0=x_0\cc{x}_K$ and $a_{2K}=\cc{a_0}$. Therefore, Huffman autocorrelations are considered as the most impulsive-like autocorrelations and generate a power spectral density (polynomial):
%
\revts $\uA(z)= -\eta + z^{K} -\eta z^{2K}$,
%
which is almost flat on the unit circle $\uA(e^{\im \nu})=1+2\eta \cos( K \nu)$.
%
Since $\eta<1/2$ the $z$-transform $\uA(z)$ has no zeros on the unit circle.  Taking $\uA(z)=0$ as a quadratic equation in $z^K$, one can immediately determine all the zeros $\alp_\nx=R_\nx e^{\im\phil}$ by
%
$R_\nx^K=R^{\pm K}= (1 \pm \sqrt{1-4\eta^2})/2\eta$ with angles $\phil= (k-1)\tht_K$, which are multiples of the
\emph{base angle} $\tht_K=2\pi/K$ for $k=1,2,\dots,K$.
%
The $K$ conjugate-reciprocal zero pairs are uniformly placed on two circles with radii $R>1$ and $R^{-1}$, i.e.,
$\alp_\nx\in\Zero_\nx=\{R e^{2\pi\im \frac{\nx-1}{K}}, R^{-1} e^{2\pi\im \frac{\nx-1}{K}}\}$.  The zeros are therefore the vertices of two regular polygons, centered at the origin, see \figref{fig:HuffmanBMOCZscheme}.  Expressing $A(z)$ by its zeros, gives
%
\begin{align}
  \uA(z) &=-\eta\Pro_{\nx=1}^K (z-\alp_\nx)
  (z-\cc{\alp_\nx^{-1}})  
  \label{eq:autohufzdomain}\\
  &  =  x_K\Pro_{\nx=1}^K (z-\alp_\nx) \cdot
  \cc{x_0} \Pro_{\nx=1}^K (z-\cc{\alp_\nx^{-1}}) =\uX(z)\cdot  z^K \cc{\uX(1/\cc{z})},\notag
\end{align}
%
where $z^K\cc{\uX(1/\cc{z})}=\sum_k \cc{x_{K-k}} z^k$ is the \emph{conjugate-reciprocal polynomial}
generated by $\cc{\xv^-}$. Each such $\uX(z)$ is called a \emph{Huffman polynomial} and their coefficients
$\xv$ a \emph{Huffman sequence}. Since the autocorrelation is  for each $\avlp\in\Zero^K$ the same,  we get with the identity
%
\begin{align}
  \Pro_{\nx=1}^K \alp_{\nx}&= \Pro_{\nx=1}^K R^{2m_\nx-1}e^{j2\pi \frac{(\nx-1)}{K}}
  =  R^{2\Norm{\vm}_0-K} e^{j2\pi \frac{\sum_{\nx=1}^{K-1} \nx}{K}}\notag\\
 &= R^{2\Norm{\vm}_0-K} e^{j2\pi  \frac{(K-1)K}{2K}}
  = R^{2\Norm{\vm}_0-K}(-1)^{K-1}
\end{align}
%
with $\cc{x_0} {x_K}\! =\!-\eta$, and $x_K(-1)^K\Pro_{\nx=1}^K \alp_\nx
=x_0$, which we obtain by comparing the coefficients with the polynomials in \eqref{eq:autohufzdomain} respectively $\uX(z)= x_K\Pro_{k=1}^K (z-\alp_k)=\sum_{k=0}^K x_k z^k$, the relation
%
\begin{align}
   &|x_0|^2 = \eta(-1)^{K\!-\!1}\Pro_\nx\alp_\nx,
 \ \ |x_K|^2 = \frac{\eta}{(-1)^{K\!-\!1}\Pro_\nx\alp_\nx}\quad\quad \notag \\
  \LRA\quad\!\!
  &x_0 \!= \!e^{j\phi_0} \sqrt{\eta} R^{\Norm{\vm}_0-\frac{K}{2}}, \ \
   x_K \!= \!-e^{j\phi_0} \! \sqrt{\eta} R^{\frac{K}{2}-\Norm{\vm}_0}
\end{align}
%
for a message $\vm=(m_1,\dots,m_K)$ with a global phase $\phi_0$.  By rewriting $\eta$ in terms of the radius $\eta =
1/(R^K+R^{-K})$ and setting $\phi_0=0$, the first and last coefficients of $\xv$ simplify to
%
\begin{align}
  x_0 =\sqrt{\frac{R^{2\Norm{\vm}_0}}{1+R^{2K}}}\ \text{ and }\
  x_K=
  -\sqrt{\frac{R^{2K-2\Norm{\vm}_0}}{1+R^{2K}}}.\label{eq:hufflastfirst}
\end{align}
%
This suggests, that \revts they \revte are dominant if $1\simeq R^K$, which will help for \emph{time synchronisation} and \emph{detection of the channel length} at the receiver \cite{WJHJ18}. Moreover, if $\vm$ is  uniformly identical distributed \revte we \revs get by the binomial theorem \revs$\Expect{|x_K|^2}=\Expect{|x_0|^2}= 2^{-K}(1+R^2)^K/(1+R^{2K})$\reve. In fact, the magnitude of the first and last coefficients can be used for \emph{parity checks}.

==> Plots_Figures/General_stuff/Frame_Comparison.tex <==
\usetikzlibrary{arrows.meta,shapes.arrows,chains,decorations.pathreplacing}

\newlength\myht
\settoheight{\myht}{$n-2$}
\tikzset{%
  MyStyle/.style={draw, text width=100pt, text height=10pt, text centered,minimum height=\myht+2*3*1mm),fill=green!20},
  MyStylef/.style={draw, text width=60pt, text height=10pt, text centered,minimum height=\myht+2*3*1mm)},
  MyStylefxn/.style={draw, text width=10pt, text height=10pt, text centered,minimum height=\myht+2*3*1mm),fill=yellow!20},
  MyStyleD/.style={draw, text width=100pt, text height=10pt, text centered,minimum height=\myht+3*2*1mm),fill=red!20},
  MyStyleDx/.style={draw, text width=25pt, text height=10pt, text centered,minimum height=\myht+3*2*1mm),fill=red!20},
  MyStyleE/.style={draw, text width=15pt, text height=10pt, text centered,minimum height=\myht+2*3*1mm),fill=yellow!20},
  MyStyleS/.style={draw, text width=40pt, text height=10pt, text centered,minimum height=\myht+2*3*1mm),,fill=red!20},
  boxy/.style = {rectangle,draw=black, minimum height=\myht+2*3*1mm ,fill=blue!20},
  boxy2/.style = {rectangle,draw=black, minimum height=\myht+2*3*1mm ,fill=red!20},
  myarrow/.style={shape=single arrow, rotate=90, inner sep=5pt, outer sep=0pt, single arrow head extend=0pt, minimum height=7.5pt, text width=0pt, draw=blue!50, fill=blue!25}
}

\begin{tikzpicture}[-{Stealth[length=2.5pt]}]

%\begin{tikzpicture}[-{Stealth[length=2.5pt]}]
    \begin{scope} [shift={(-4,-2.5)},name=scope1,start chain, node distance=-.5pt]
    \foreach \name [count=\xi] in {1}{ \node[MyStyle, on chain] (vlosI\xi) {STF};}
     \foreach \name [count=\xi] in {1}{ \node[MyStyle, on chain] (vlosfI\xi) {CEF};}
     \foreach \name [count=\xi] in {1}{ \node[MyStylef, on chain] (vlosgI\xi) {Header};}
     \foreach \name [count=\xi] in {1}{ \node[MyStyleD, on chain] (vlosDI\xi) {Data Blocks (BLK)};}
     \foreach \name [count=\xi] in {1}{ \node[boxy, on chain] (vlosEI\xi) {OS};}
  \end{scope}

    %   \node[above= 0.1cm of vlosI1, xshift=-0.0cm]{$T_{FB,SP}$};
    % \node[above= 0.1cm of vlosDI1, xshift=-0.5cm]{$T_{DL}$};
    % \node[above= 0.1cm of vlosEI1, xshift=0.0cm]{$T_{SP}$};
      \draw [decorate,decoration={brace,amplitude=10pt,mirror}]
  (vlosI1.south west) -- (vlosfI1.south east) node[black,midway,below=8pt]
  {Preamble};

  
  \begin{scope} [shift={(-4.0,-5)}, start chain, node distance=-.5pt]
    \foreach \name [count=\xi] in {2}{ \node[MyStyleDx, on chain] (vlosfS\xi) {BLK};}
    \foreach \name [count=\xi] in {2}{ \node[MyStyleDx, on chain] (vlosfS1\xi) {...};}
     \foreach \name [count=\xi] in {2}{ \node[MyStyleDx, on chain] (vlosDS\xi) {BLK};}
     \foreach \name [count=\xi] in {2}{ \node[MyStylefxn, on chain] (vlosFxn\xi) {};}
     
     \foreach \name [count=\xi] in {2}{ \node[MyStyleDx, on chain] (vlosf2S\xi) {BLK};}
     \foreach \name [count=\xi] in {2}{ \node[MyStyleDx, on chain] (vlosf2S1\xi) {...};}
     \foreach \name [count=\xi] in {2}{ \node[MyStyleDx, on chain] (vlosD2S\xi) {BLK};}
     \foreach \name [count=\xi] in {2}{ \node[MyStylefxn, on chain] (vlosFxn2\xi) {};}
     
    \foreach \name [count=\xi] in {2}{ \node[MyStyleDx, on chain] (vlosf3S\xi) {BLK};}
    \foreach \name [count=\xi] in {2}{ \node[MyStyleDx, on chain] (vlosf3S1\xi) {...};}
     \foreach \name [count=\xi] in {2}{ \node[MyStyleDx, on chain] (vlosD3S\xi) {BLK};}
  \end{scope}
    % \node[above= 0.1cm of vlosf1, xshift=-0.0cm]{$T_{FB,SP}$};
    % \node[above= 0.1cm of vlosD1, xshift=-0.5cm]{$T_{DL}$};
    % \node[above= 0.1cm of vlosE1, xshift=0.0cm]{$T_{SP}$};
    \node[right = 0.25cm of vlosD3S1, xshift=0.0cm]{\LARGE $\cdot\cdots$};
    
      \draw [decorate,decoration={brace,amplitude=10pt,mirror}]
  (vlosfS1.south west) -- (vlosDS1.south east) node[black,midway,below=12pt]
  {$\Omega_1$: T$_{CPI}$};

    \draw [decorate,decoration={brace,amplitude=8pt,mirror}]
  (vlosDS1.south east) -- (vlosf2S1.south west) node[black,midway,below=10pt]
  {T$_{swc}$};

  
    \draw [decorate,decoration={brace,amplitude=10pt,mirror}]
  (vlosf2S1.south west) -- (vlosD2S1.south east) node[black,midway,below=12pt]
  {$\Omega_2$: T$_{CPI}$};

    \draw [decorate,decoration={brace,amplitude=8pt,mirror}]
  (vlosD2S1.south east) -- (vlosf3S1.south west) node[black,midway,below=10pt]
  {T$_{swc}$};

    \draw [decorate,decoration={brace,amplitude=10pt,mirror}]
  (vlosf3S1.south west) -- (vlosD3S1.south east) node[black,midway,below=12pt]
  {$\Omega_3$: T$_{CPI}$};
  
  %\node[draw] at (-7, 0)   (a) {(a)};
  \node[] at (-7, -2.5)   (b) {\Large (a)};
  \node[] at (-7, -5)   (a) {\Large (b)};
%  \draw [decorate,decoration={brace,amplitude=10pt,mirror}]
%  (vlos7.south west) -- (vlos11.south east) node[black,midway,below=8pt]
%  {Removed data};
\end{tikzpicture}

